ScriptNet: Neural Static Analysis for Malicious JavaScript Detection

Malicious scripts are an important computer infection threat vector in the wild. For web-scale processing, static analysis offers substantial computing efficiencies. We propose the ScriptNet system for neural malicious JavaScript detection which is based on static analysis. We use the Convoluted Partitioning of Long Sequences (CPoLS) model, which processes Javascript files as byte sequences. Lower layers capture the sequential nature of these byte sequences while higher layers classify the resulting embedding as malicious or benign. Unlike previously proposed solutions, our model variants are trained in an end-to-end fashion allowing discriminative training even for the sequential processing layers. Evaluating this model on a large corpus of 212,408 JavaScript files indicates that the best performing CPoLS model offers a 97.20% true positive rate (TPR) for the first 60K byte subsequence at a false positive rate (FPR) of 0.50%. The best performing CPoLS model significantly outperform several baseline models.

==> figs/BASELINE_LR_comp_results_header.tex <==
$\textsc{LR - Trigram}$ $(L_{LR}=1, C_{LR}=1, T=1000)$ & 97.5975 & 97.9394 & 99.3477 & 0.9864 & 0.9237 \\


==> figs/BASELINE_LR_comp_results_header2.tex <==
$\textsc{LR - Trigram}$ $(L_{LR}=1, C_{LR}=1, T=1000)$ & 97.5975 & 97.9394 & 99.3477 & 99.3284 & 0.9864 & 0.9237 \\


==> figs/JS_BASELINE_80K_071918_comp_results_header2.tex <==
$\textsc{SdA-LR}$ $(T=2000)$ & 87.6020 & 87.6020 & 100.0000 & 0.5296 & 0.9339 & 0.5012 \\
$\textsc{KOL-CNN}$ $(T=200)$ & 97.0753 & 97.4956 & 99.2097 & 71.6832 & 0.9835 & 0.9853 \\
$\textsc{KOL-CNN}$ $(T=1000)$ & 96.7446 & 96.8356 & 99.5363 & 37.6286 & 0.9817 & 0.9851 \\
$\textsc{LR - Trigram}$ $(T=60K)$ & 97.5975 & 97.9394 & 99.3477 & 99.3284 & 0.9864 & 0.9237 \\
$\textsc{SVM - Trigram}$ $(T=60K)$ & 97.5560 & 97.7683 & 99.4810 & 99.4704 & 0.9862 & 0.9185 \\


==> figs/JS_FINAL_ARX_COMP_80K_071918_comp_results_header.tex <==
$\textsc{CPoLS-LSTM-NN}$ $(L=1, C=2, T=60K)$ & 98.9708 & 99.1626 & 99.6668 & 0.9941 & 0.9984 \\
$\textsc{CPoLS-BiLSTM-NN}$ $(L=2, C=1, T=60K)$ & 99.1398 & 99.2981 & 99.7229 & 0.9951 & 0.9986 \\
$\textsc{LaMP-LSTM-NN}$ $(L=2, C=1, T=200)$ & 96.3953 & 96.4409 & 99.5592 & 0.9798 & 0.9873 \\
$\textsc{KOL-CNN}$ $(T=200)$ & 97.0753 & 97.4956 & 99.2097 & 0.9835 & 0.9853 \\
$\textsc{SdA-LR}$ $(T=2000)$ & 87.6020 & 87.6020 & 100.0000 & 0.9339 & 0.5012 \\


==> figs/JS_FINAL_ARX_COMP_80K_071918_comp_results_header2.tex <==
$\textsc{CPoLS-LSTM-NN}$ $(L=1, C=2, T=60K)$ & 98.9708 & 99.1626 & 99.6668 & 95.0498 & 0.9941 & 0.9984 \\
$\textsc{CPoLS-BiLSTM-NN}$ $(L=2, C=1, T=60K)$ & 99.1398 & 99.2981 & 99.7229 & 97.2049 & 0.9951 & 0.9986 \\
$\textsc{LaMP-LSTM-NN}$ $(L=2, C=1, T=200)$ & 96.3953 & 96.4409 & 99.5592 & 70.3853 & 0.9798 & 0.9873 \\
$\textsc{KOL-CNN}$ $(T=200)$ & 97.0753 & 97.4956 & 99.2097 & 71.6832 & 0.9835 & 0.9853 \\
$\textsc{SdA-LR}$ $(T=2000)$ & 87.6020 & 87.6020 & 100.0000 & 0.5296 & 0.9339 & 0.5012 \\


==> figs/JS_FINAL_COMP_80K_071918_comp_results_header.tex <==
$\textsc{PIL-LSTM-NN}$ $(L=1, C=1, T=60K)$ & 98.6236 & 98.5739 & 99.8737 & 0.9922 & 0.9988 \\
$\textsc{PIL-BiLSTM-NN}$ $(L=1, C=1, T=60K)$ & 99.4577 & 99.6896 & 99.6914 & 0.9969 & 0.9984 \\
$\textsc{CPoLS-LSTM-NN}$ $(L=1, C=2, T=60K)$ & 98.9708 & 99.1626 & 99.6668 & 0.9941 & 0.9984 \\
$\textsc{CPoLS-BiLSTM-NN}$ $(L=2, C=1, T=60K)$ & 99.1398 & 99.2981 & 99.7229 & 0.9951 & 0.9986 \\
$\textsc{LaMP-LSTM-NN}$ $(L=2, C=1, T=200)$ & 96.3953 & 96.4409 & 99.5592 & 0.9798 & 0.9873 \\
$\textsc{KOL-CNN}$ $(T=200)$ & 97.0753 & 97.4956 & 99.2097 & 0.9835 & 0.9853 \\


==> figs/JS_FINAL_COMP_80K_071918_comp_results_header2.tex <==
$\textsc{PIL-LSTM-NN}$ $(L=1, C=1, T=60K)$ & 98.6236 & 98.5739 & 99.8737 & 98.1027 & 0.9922 & 0.9988 \\
$\textsc{PIL-BiLSTM-NN}$ $(L=1, C=1, T=60K)$ & 99.4577 & 99.6896 & 99.6914 & 97.5819 & 0.9969 & 0.9984 \\
$\textsc{CPoLS-LSTM-NN}$ $(L=1, C=2, T=60K)$ & 98.9708 & 99.1626 & 99.6668 & 95.0498 & 0.9941 & 0.9984 \\
$\textsc{CPoLS-BiLSTM-NN}$ $(L=2, C=1, T=60K)$ & 99.1398 & 99.2981 & 99.7229 & 97.2049 & 0.9951 & 0.9986 \\
$\textsc{LaMP-LSTM-NN}$ $(L=2, C=1, T=200)$ & 96.3953 & 96.4409 & 99.5592 & 70.3853 & 0.9798 & 0.9873 \\
$\textsc{KOL-CNN}$ $(T=200)$ & 97.0753 & 97.4956 & 99.2097 & 71.6832 & 0.9835 & 0.9853 \\


==> figs/JS_MPL_80K_052418_comp_results_header.tex <==
$\textsc{LaMP}$ $(L_{LaMP}=1, C_{LaMP}=1, T=200)$ & 96.2908 & 96.7896 & 97.4896 & 0.9714 & 0.9933 \\
$\textsc{LaMP}$ $(L_{LaMP}=1, C_{LaMP}=2, T=200)$ & 95.7421 & 97.1555 & 96.2234 & 0.9669 & 0.9906 \\
$\textsc{LaMP}$ $(L_{LaMP}=2, C_{LaMP}=1, T=200)$ & 87.3929 & 87.8721 & 93.3624 & 0.9053 & 0.9155 \\
$\textsc{LaMP}$ $(L_{LaMP}=2, C_{LaMP}=2, T=200)$ & 94.1398 & 93.3262 & 97.9279 & 0.9557 & 0.9880 \\


==> figs/JS_MPL_80K_071918_comp_results_header2.tex <==
$\textsc{LaMP-LSTM-LR}$ $(L=1, C=0, T=200)$ & 95.9861 & 96.6608 & 98.8321 & 33.4610 & 0.9773 & 0.9766 \\
$\textsc{LaMP-LSTM-NN}$ $(L=1, C=1, T=200)$ & 97.0138 & 96.9490 & 99.7295 & 80.1697 & 0.9832 & 0.9892 \\
$\textsc{LaMP-LSTM-DNN}$ $(L=1, C=2, T=200)$ & 96.3953 & 96.4409 & 99.5592 & 70.3853 & 0.9798 & 0.9873 \\
$\textsc{LaMP-LSTM-LR}$ $(L=2, C=0, T=200)$ & 87.5983 & 87.5983 & 100.0000 & 100.0000 & 0.9339 & 0.5000 \\
$\textsc{LaMP-LSTM-NN}$ $(L=2, C=1, T=200)$ & 94.1814 & 96.0273 & 97.3866 & 9.4383 & 0.9670 & 0.9500 \\
$\textsc{LaMP-LSTM-DNN}$ $(L=2, C=2, T=200)$ & 96.1169 & 97.8491 & 97.7151 & 29.8816 & 0.9778 & 0.9748 \\


==> figs/JS_MPL_comp_results_header.tex <==
$\textsc{LaMP-LSTM-NN}$ $(L=1, C=1, T=200)$ & 92.0066 & 90.6938 & 95.6187 & 0.9309 & 0.9706 \\
$\textsc{LaMP-LSTM-DNN}$ $(L=1, C=2, T=200)$ & 95.2877 & 93.5037 & 98.4746 & 0.9592 & 0.9852 \\
$\textsc{LaMP-LSTM-NN}$ $(L=2, C=1, T=200)$ & 95.0970 & 93.3515 & 98.2948 & 0.9576 & 0.9849 \\
$\textsc{LaMP-LSTM-DNN}$ $(L=2, C=2, T=200)$ & 93.3805 & 92.7723 & 95.7026 & 0.9421 & 0.9776 \\


==> figs/JS_MPL_comp_results_header2.tex <==
$\textsc{LaMP-LSTM-NN}$ $(L=1, C=1, T=200)$ & 92.0066 & 90.6938 & 95.6187 & 32.6650 & 0.9309 & 0.9706 \\
$\textsc{LaMP-LSTM-DNN}$ $(L=1, C=2, T=200)$ & 95.2877 & 93.5037 & 98.4746 & 48.5690 & 0.9592 & 0.9852 \\
$\textsc{LaMP-LSTM-NN}$ $(L=2, C=1, T=200)$ & 95.0970 & 93.3515 & 98.2948 & 43.4145 & 0.9576 & 0.9849 \\
$\textsc{LaMP-LSTM-DNN}$ $(L=2, C=2, T=200)$ & 93.3805 & 92.7723 & 95.7026 & 33.3633 & 0.9421 & 0.9776 \\


==> figs/JS_NB_COMP_80K_071918_comp_results_header2.tex <==
$\textsc{NB - Trigram}$ $(T=60K)$ & 97.5560 & 97.7683 & 99.4810 & 99.4704 & 0.9862 & 0.9185 \\


==> figs/JS_PIL_80K_052418_hidden_comp_results_header.tex <==
$\textsc{PIL}$ $(L_{PIL}=1, C_{PIL}=1, T=80000)$ & 98.8053 & 98.7914 & 99.3654 & 0.9908 & 0.9978 \\
$\textsc{PIL}$ $(L_{PIL}=1, C_{PIL}=2, T=80000)$ & 98.9293 & 99.2020 & 99.1393 & 0.9917 & 0.9984 \\
$\textsc{PIL}$ $(L_{PIL}=2, C_{PIL}=1, T=80000)$ & 98.9419 & 99.0780 & 99.2852 & 0.9918 & 0.9984 \\
$\textsc{PIL}$ $(L_{PIL}=2, C_{PIL}=2, T=80000)$ & 98.8116 & 98.8907 & 99.2730 & 0.9908 & 0.9984 \\


==> figs/JS_PIL_80K_071918_comp_results_header.tex <==
$\textsc{PIL-LSTM-LR}$ $(L=1, C=0, T=60K)$ & 98.3395 & 98.4515 & 99.6721 & 0.9906 & 0.9968 \\
$\textsc{PIL-LSTM-NN}$ $(L=1, C=1, T=60K)$ & 98.6236 & 98.5739 & 99.8737 & 0.9922 & 0.9988 \\
$\textsc{PIL-LSTM-DNN}$ $(L=1, C=2, T=60K)$ & 99.0092 & 99.1269 & 99.7475 & 0.9944 & 0.9980 \\
$\textsc{PIL-LSTM-LR}$ $(L=2, C=0, T=60K)$ & 98.8372 & 98.9373 & 99.7440 & 0.9934 & 0.9984 \\
$\textsc{PIL-LSTM-NN}$ $(L=2, C=1, T=60K)$ & 98.8541 & 98.8899 & 99.8124 & 0.9935 & 0.9986 \\
$\textsc{PIL-LSTM-DNN}$ $(L=2, C=2, T=60K)$ & 99.0799 & 99.2993 & 99.6528 & 0.9948 & 0.9983 \\


==> figs/JS_PIL_80K_071918_comp_results_header2.tex <==
$\textsc{PIL-LSTM-LR}$ $(L=1, C=0, T=60K)$ & 98.3395 & 98.4515 & 99.6721 & 93.3997 & 0.9906 & 0.9968 \\
$\textsc{PIL-LSTM-NN}$ $(L=1, C=1, T=60K)$ & 98.6236 & 98.5739 & 99.8737 & 98.1027 & 0.9922 & 0.9988 \\
$\textsc{PIL-LSTM-DNN}$ $(L=1, C=2, T=60K)$ & 99.0092 & 99.1269 & 99.7475 & 95.3865 & 0.9944 & 0.9980 \\
$\textsc{PIL-LSTM-LR}$ $(L=2, C=0, T=60K)$ & 98.8372 & 98.9373 & 99.7440 & 96.7192 & 0.9934 & 0.9984 \\
$\textsc{PIL-LSTM-NN}$ $(L=2, C=1, T=60K)$ & 98.8541 & 98.8899 & 99.8124 & 97.2575 & 0.9935 & 0.9986 \\
$\textsc{PIL-LSTM-DNN}$ $(L=2, C=2, T=60K)$ & 99.0799 & 99.2993 & 99.6528 & 93.2489 & 0.9948 & 0.9983 \\


==> figs/JS_PIL_80K_071918_comp_results_header_100.tex <==
$\textsc{PIL-LSTM-LR}$ $(L=1, C=0, T=60K)$ & 98.3395 & 98.4515 & 99.6721 & 0.9906 & 0.9968 \\
$\textsc{PIL-LSTM-NN}$ $(L=1, C=1, T=60K)$ & 98.6236 & 98.5739 & 99.8737 & 0.9922 & 0.9988 \\
$\textsc{PIL-LSTM-DNN}$ $(L=1, C=2, T=60K)$ & 99.0092 & 99.1269 & 99.7475 & 0.9944 & 0.9980 \\
$\textsc{PIL-LSTM-LR}$ $(L=2, C=0, T=60K)$ & 98.8372 & 98.9373 & 99.7440 & 0.9934 & 0.9984 \\
$\textsc{PIL-LSTM-NN}$ $(L=2, C=1, T=60K)$ & 98.8541 & 98.8899 & 99.8124 & 0.9935 & 0.9986 \\
$\textsc{PIL-LSTM-DNN}$ $(L=2, C=2, T=60K)$ & 99.0799 & 99.2993 & 99.6528 & 0.9948 & 0.9983 \\


==> figs/JS_PIL_80K_071918_comp_results_header_1002.tex <==
$\textsc{PIL-LSTM-LR}$ $(L=1, C=0, T=60K)$ & 98.3395 & 98.4515 & 99.6721 & 93.3997 & 0.9906 & 0.9968 \\
$\textsc{PIL-LSTM-NN}$ $(L=1, C=1, T=60K)$ & 98.6236 & 98.5739 & 99.8737 & 98.1027 & 0.9922 & 0.9988 \\
$\textsc{PIL-LSTM-DNN}$ $(L=1, C=2, T=60K)$ & 99.0092 & 99.1269 & 99.7475 & 95.3865 & 0.9944 & 0.9980 \\
$\textsc{PIL-LSTM-LR}$ $(L=2, C=0, T=60K)$ & 98.8372 & 98.9373 & 99.7440 & 96.7192 & 0.9934 & 0.9984 \\
$\textsc{PIL-LSTM-NN}$ $(L=2, C=1, T=60K)$ & 98.8541 & 98.8899 & 99.8124 & 97.2575 & 0.9935 & 0.9986 \\
$\textsc{PIL-LSTM-DNN}$ $(L=2, C=2, T=60K)$ & 99.0799 & 99.2993 & 99.6528 & 93.2489 & 0.9948 & 0.9983 \\


==> figs/JS_PIL_BILSTM_80K_071918_comp_results_header.tex <==
$\textsc{PIL-BiLSTM-LR}$ $(L=1, C=0, T=60K)$ & 99.0399 & 99.1649 & 99.7440 & 0.9945 & 0.9979 \\
$\textsc{PIL-BiLSTM-NN}$ $(L=1, C=1, T=60K)$ & 99.4577 & 99.6896 & 99.6914 & 0.9969 & 0.9984 \\
$\textsc{PIL-BiLSTM-DNN}$ $(L=1, C=2, T=60K)$ & 97.5914 & 97.3677 & 99.9527 & 0.9864 & 0.9977 \\
$\textsc{PIL-BiLSTM-LR}$ $(L=2, C=0, T=60K)$ & 98.6774 & 98.6556 & 99.8510 & 0.9925 & 0.9979 \\
$\textsc{PIL-BiLSTM-NN}$ $(L=2, C=1, T=60K)$ & 99.3241 & 99.5187 & 99.7107 & 0.9961 & 0.9989 \\
$\textsc{PIL-BiLSTM-DNN}$ $(L=2, C=2, T=60K)$ & 99.0937 & 99.1500 & 99.8211 & 0.9948 & 0.9985 \\


==> figs/JS_PIL_BILSTM_80K_071918_comp_results_header2.tex <==
$\textsc{PIL-BiLSTM-LR}$ $(L=1, C=0, T=60K)$ & 99.0399 & 99.1649 & 99.7440 & 95.2269 & 0.9945 & 0.9979 \\
$\textsc{PIL-BiLSTM-NN}$ $(L=1, C=1, T=60K)$ & 99.4577 & 99.6896 & 99.6914 & 97.5819 & 0.9969 & 0.9984 \\
$\textsc{PIL-BiLSTM-DNN}$ $(L=1, C=2, T=60K)$ & 97.5914 & 97.3677 & 99.9527 & 96.9734 & 0.9864 & 0.9977 \\
$\textsc{PIL-BiLSTM-LR}$ $(L=2, C=0, T=60K)$ & 98.6774 & 98.6556 & 99.8510 & 90.5923 & 0.9925 & 0.9979 \\
$\textsc{PIL-BiLSTM-NN}$ $(L=2, C=1, T=60K)$ & 99.3241 & 99.5187 & 99.7107 & 97.2435 & 0.9961 & 0.9989 \\
$\textsc{PIL-BiLSTM-DNN}$ $(L=2, C=2, T=60K)$ & 99.0937 & 99.1500 & 99.8211 & 97.9712 & 0.9948 & 0.9985 \\


==> figs/JS_PIL_CHUNKED_FULL_071918_comp_results_header.tex <==
$\textsc{PIL-LSTM-NN}$ $(L=1, C=1, R=200, T=60K)$ & 98.6236 & 98.5739 & 99.8737 & 0.9922 & 0.9988 \\
$\textsc{PIL-LSTM-NN}$ $(L=1, C=1, R=200, T=Full)$ & 97.4288 & 97.5455 & 99.5704 & 0.9855 & 0.9916 \\
$\textsc{PIL-LSTM-NN}$ $(L=1, C=1, R=50, T=Full)$ & 96.7315 & 96.6968 & 99.6739 & 0.9816 & 0.9922 \\


==> figs/JS_PIL_CHUNKED_FULL_071918_comp_results_header2.tex <==
$\textsc{PIL-LSTM-NN}$ $(L=1, C=1, R=200, T=60K)$ & 98.6236 & 98.5739 & 99.8737 & 98.1027 & 0.9922 & 0.9988 \\
$\textsc{PIL-LSTM-NN}$ $(L=1, C=1, R=200, T=Full)$ & 97.4288 & 97.5455 & 99.5704 & 81.6621 & 0.9855 & 0.9916 \\
$\textsc{PIL-LSTM-NN}$ $(L=1, C=1, R=50, T=Full)$ & 96.7315 & 96.6968 & 99.6739 & 80.7785 & 0.9816 & 0.9922 \\


==> figs/JS_PIL_CHUNKED_FULL_071918_comp_results_header_2.tex <==
$\textsc{PIL-LSTM-NN}$ $(L=1, C=1, R=200, T=Full)$ & 97.4288 & 97.5455 & 99.5704 & 0.9855 & 0.9916 \\
$\textsc{PIL-LSTM-NN}$ $(L=1, C=1, R=50, T=Full)$ & 96.7315 & 96.6968 & 99.6739 & 0.9816 & 0.9922 \\


==> figs/JS_PIL_CHUNKED_FULL_071918_comp_results_header_22.tex <==
$\textsc{PIL-LSTM-NN}$ $(L=1, C=1, R=200, T=Full)$ & 97.4288 & 97.5455 & 99.5704 & 81.6621 & 0.9855 & 0.9916 \\
$\textsc{PIL-LSTM-NN}$ $(L=1, C=1, R=50, T=Full)$ & 96.7315 & 96.6968 & 99.6739 & 80.7785 & 0.9816 & 0.9922 \\


==> figs/JS_SCL_80K_052418_hidden_comp_results_header.tex <==
$\textsc{CPoLS-LogReg}$ $(L_{CPoLS}=1, C_{CPoLS}=0, T=80000)$ & 98.6091 & 99.3791 & 98.4610 & 0.9892 & 0.9983 \\
$\textsc{CPoLS}$ $(L_{CPoLS}=1, C_{CPoLS}=1, T=80000)$ & 98.8760 & 98.7762 & 99.4919 & 0.9913 & 0.9983 \\
$\textsc{CPoLS}$ $(L_{CPoLS}=1, C_{CPoLS}=2, T=80000)$ & 98.7802 & 99.2506 & 98.8573 & 0.9905 & 0.9985 \\
$\textsc{CPoLS}$ $(L_{CPoLS}=1, C_{CPoLS}=3, T=80000)$ & 98.7205 & 98.5664 & 99.4651 & 0.9901 & 0.9982 \\
$\textsc{CPoLS}$ $(L_{CPoLS}=1, C_{CPoLS}=4, T=80000)$ & 98.7849 & 98.5772 & 99.5551 & 0.9906 & 0.9980 \\


==> figs/JS_SCL_80K_071918_comp_results_header2.tex <==
$\textsc{CPoLS-LSTM-LR}$ $(L=1, C=0, T=60K)$ & 98.8725 & 98.9990 & 99.7212 & 96.1230 & 0.9936 & 0.9985 \\
$\textsc{CPoLS-LSTM-NN}$ $(L=1, C=1, T=60K)$ & 98.1997 & 98.2232 & 99.7492 & 68.7802 & 0.9898 & 0.9937 \\
$\textsc{CPoLS-LSTM-DNN}$ $(L=1, C=2, T=60K)$ & 98.1966 & 98.1135 & 99.8615 & 85.4089 & 0.9898 & 0.9964 \\
$\textsc{CPoLS-LSTM-LR}$ $(L=2, C=0, T=60K)$ & 99.0399 & 99.3888 & 99.5160 & 94.0117 & 0.9945 & 0.9975 \\
$\textsc{CPoLS-LSTM-NN}$ $(L=2, C=1, T=60K)$ & 98.9708 & 99.1626 & 99.6668 & 95.0498 & 0.9941 & 0.9984 \\
$\textsc{CPoLS-LSTM-DNN}$ $(L=2, C=2, T=60K)$ & 98.8771 & 99.1909 & 99.5301 & 94.5080 & 0.9936 & 0.9981 \\


==> figs/JS_SCL_80K_071918_hidden_comp_results_header.tex <==
$\textsc{CPoLS-LSTM-LR}$ $(L=1, C=0, T=60K)$ & 98.8725 & 98.9990 & 99.7212 & 0.9936 & 0.9985 \\
$\textsc{CPoLS-LSTM-NN}$ $(L=1, C=1, T=60K)$ & 98.1997 & 98.2232 & 99.7492 & 0.9898 & 0.9937 \\
$\textsc{CPoLS-LSTM-DNN}$ $(L=1, C=2, T=60K)$ & 98.1966 & 98.1135 & 99.8615 & 0.9898 & 0.9964 \\
$\textsc{CPoLS-LSTM-DNN}$ $(L=1, C=3, T=60K)$ & 98.3809 & 98.4254 & 99.7475 & 0.9908 & 0.9951 \\
$\textsc{CPoLS-LSTM-DNN}$ $(L=1, C=4, T=60K)$ & 98.1935 & 98.2631 & 99.7001 & 0.9898 & 0.9954 \\


==> figs/JS_SCL_80K_071918_hidden_comp_results_header2.tex <==
$\textsc{CPoLS-LSTM-LR}$ $(L=1, C=0, T=60K)$ & 98.8725 & 98.9990 & 99.7212 & 96.1230 & 0.9936 & 0.9985 \\
$\textsc{CPoLS-LSTM-NN}$ $(L=1, C=1, T=60K)$ & 98.1997 & 98.2232 & 99.7492 & 68.7802 & 0.9898 & 0.9937 \\
$\textsc{CPoLS-LSTM-DNN}$ $(L=1, C=2, T=60K)$ & 98.1966 & 98.1135 & 99.8615 & 85.4089 & 0.9898 & 0.9964 \\
$\textsc{CPoLS-LSTM-DNN}$ $(L=1, C=3, T=60K)$ & 98.3809 & 98.4254 & 99.7475 & 77.4812 & 0.9908 & 0.9951 \\
$\textsc{CPoLS-LSTM-DNN}$ $(L=1, C=4, T=60K)$ & 98.1935 & 98.2631 & 99.7001 & 78.6824 & 0.9898 & 0.9954 \\


==> figs/JS_SCL_80K_comp_results_header.tex <==
$\textsc{CPoLS-LSTM-NN}$ $(L=1, C=1, T=60K)$ & 98.8760 & 98.7762 & 99.4919 & 0.9913 & 0.9983 \\
$\textsc{CPoLS-LSTM-DNN}$ $(L=1, C=2, T=60K)$ & 98.7802 & 99.2506 & 98.8573 & 0.9905 & 0.9985 \\
$\textsc{CPoLS-LSTM-NN}$ $(L=2, C=1, T=60K)$ & 98.8571 & 98.8466 & 99.3897 & 0.9912 & 0.9983 \\
$\textsc{CPoLS-LSTM-DNN}$ $(L=2, C=2, T=60K)$ & 98.2574 & 97.8388 & 99.4991 & 0.9866 & 0.9976 \\


==> figs/JS_SCL_80K_comp_results_header2.tex <==
$\textsc{CPoLS-LSTM-NN}$ $(L=1, C=1, T=60K)$ & 98.8760 & 98.7762 & 99.4919 & 94.4444 & 0.9913 & 0.9983 \\
$\textsc{CPoLS-LSTM-DNN}$ $(L=1, C=2, T=60K)$ & 98.7802 & 99.2506 & 98.8573 & 95.1179 & 0.9905 & 0.9985 \\
$\textsc{CPoLS-LSTM-NN}$ $(L=2, C=1, T=60K)$ & 98.8571 & 98.8466 & 99.3897 & 94.8067 & 0.9912 & 0.9983 \\
$\textsc{CPoLS-LSTM-DNN}$ $(L=2, C=2, T=60K)$ & 98.2574 & 97.8388 & 99.4991 & 91.8332 & 0.9866 & 0.9976 \\


==> figs/JS_SCL_BILSTM_80K_071918_comp_results_header2.tex <==
$\textsc{CPoLS-BiLSTM-LR}$ $(L=1, C=0, T=60K)$ & 98.5683 & 98.5394 & 99.8457 & 84.2481 & 0.9919 & 0.9967 \\
$\textsc{CPoLS-BiLSTM-NN}$ $(L=1, C=1, T=60K)$ & 98.6928 & 98.7318 & 99.7896 & 83.4152 & 0.9926 & 0.9956 \\
$\textsc{CPoLS-BiLSTM-DNN}$ $(L=1, C=2, T=60K)$ & 98.7035 & 98.8149 & 99.7159 & 85.2388 & 0.9926 & 0.9969 \\
$\textsc{CPoLS-BiLSTM-LR}$ $(L=2, C=0, T=60K)$ & 98.7988 & 98.8773 & 99.7615 & 96.5157 & 0.9932 & 0.9982 \\
$\textsc{CPoLS-BiLSTM-NN}$ $(L=2, C=1, T=60K)$ & 99.1398 & 99.2981 & 99.7229 & 97.2049 & 0.9951 & 0.9986 \\
$\textsc{CPoLS-BiLSTM-DNN}$ $(L=2, C=2, T=60K)$ & 97.5530 & 97.4753 & 99.7913 & 84.6777 & 0.9862 & 0.9969 \\


==> figs/JS_SCL_BILSTM_80K_071918_hidden_comp_results_header.tex <==
$\textsc{CPoLS, BILSTM}$ $(L_{CPoLS, BILSTM}=1, C_{CPoLS,BILSTM}=1, T=80000)$ & 98.6928 & 98.7318 & 99.7896 & 0.9926 & 0.9956 \\
$\textsc{CPoLS, BILSTM}$ $(L_{CPoLS, BILSTM}=1, C_{CPoLS,BILSTM}=2, T=80000)$ & 98.7035 & 98.8149 & 99.7159 & 0.9926 & 0.9969 \\
$\textsc{CPoLS, BILSTM}$ $(L_{CPoLS, BILSTM}=2, C_{CPoLS,BILSTM}=1, T=80000)$ & 99.1398 & 99.2981 & 99.7229 & 0.9951 & 0.9986 \\
$\textsc{CPoLS, BILSTM}$ $(L_{CPoLS, BILSTM}=2, C_{CPoLS,BILSTM}=2, T=80000)$ & 97.5530 & 97.4753 & 99.7913 & 0.9862 & 0.9969 \\


==> figs/JS_SCL_comp_results_header.tex <==
$\textsc{CPoLS-LSTM}$ $(L=1, C=1, T=1000)$ & 95.0345 & 96.2909 & 94.8365 & 0.9556 & 0.9829 \\
$\textsc{CPoLS-LSTM}$ $(L=1, C=2, T=1000)$ & 95.5932 & 95.7545 & 96.4518 & 0.9610 & 0.9823 \\
$\textsc{CPoLS-LSTM}$ $(L=2, C=1, T=1000)$ & 95.1442 & 93.2143 & 98.5525 & 0.9581 & 0.9780 \\
$\textsc{CPoLS-LSTM}$ $(L=2, C=2, T=1000)$ & 95.0953 & 93.7322 & 97.8333 & 0.9574 & 0.9793 \\


==> figs/JS_SCL_comp_results_header2.tex <==
$\textsc{CPoLS-LSTM}$ $(L=1, C=1, T=1000)$ & 95.0345 & 96.2909 & 94.8365 & 31.8379 & 0.9556 & 0.9829 \\
$\textsc{CPoLS-LSTM}$ $(L=1, C=2, T=1000)$ & 95.5932 & 95.7545 & 96.4518 & 30.2436 & 0.9610 & 0.9823 \\
$\textsc{CPoLS-LSTM}$ $(L=2, C=1, T=1000)$ & 95.1442 & 93.2143 & 98.5525 & 30.1567 & 0.9581 & 0.9780 \\
$\textsc{CPoLS-LSTM}$ $(L=2, C=2, T=1000)$ & 95.0953 & 93.7322 & 97.8333 & 30.6362 & 0.9574 & 0.9793 \\


==> figs/VBS_MPL_comp_results_header.tex <==
$\textsc{VBS}$ $(L_{VBS,LaMP}=1, C_{VBS,LaMP}=1, T=200)$ & 93.2493 & 91.6020 & 83.0611 & 0.8712 & 0.9773 \\
$\textsc{VBS}$ $(L_{VBS,LaMP}=1, C_{VBS,LaMP}=2, T=200)$ & 89.5736 & 88.8794 & 70.9543 & 0.7891 & 0.9529 \\
$\textsc{VBS}$ $(L_{VBS,LaMP}=2, C_{VBS,LaMP}=1, T=200)$ & 91.3241 & 84.4537 & 83.8854 & 0.8417 & 0.9616 \\
$\textsc{VBS}$ $(L_{VBS,LaMP}=2, C_{VBS,LaMP}=2, T=200)$ & 85.4051 & 66.6954 & 93.7084 & 0.7793 & 0.9584 \\


==> figs/VBS_SCL_comp_results_header.tex <==
$\textsc{VBS}$ $(L_{VBS,CPoLS}=1, C_{VBS,CPoLS}=1, T=1000)$ & 92.7712 & 85.2208 & 89.1712 & 0.8715 & 0.9681 \\
$\textsc{VBS}$ $(L_{VBS,CPoLS}=1, C_{VBS,CPoLS}=2, T=1000)$ & 92.1433 & 82.2465 & 91.0844 & 0.8644 & 0.9714 \\
$\textsc{VBS}$ $(L_{VBS,CPoLS}=2, C_{VBS,CPoLS}=1, T=1000)$ & 93.2265 & 88.1547 & 87.0614 & 0.8760 & 0.9730 \\
$\textsc{VBS}$ $(L_{VBS,CPoLS}=2, C_{VBS,CPoLS}=2, T=1000)$ & 93.2473 & 89.4059 & 85.5792 & 0.8745 & 0.9706 \\


==> figs/VBS_SCL_comp_results_header2.tex <==
$\textsc{VBS}$ $(L_{VBS,CPoLS}=1, C_{VBS,CPoLS}=1, T=1000)$ & 92.7712 & 85.2208 & 89.1712 & 58.1292 & 0.8715 & 0.9681 \\
$\textsc{VBS}$ $(L_{VBS,CPoLS}=1, C_{VBS,CPoLS}=2, T=1000)$ & 92.1433 & 82.2465 & 91.0844 & 54.2801 & 0.8644 & 0.9714 \\
$\textsc{VBS}$ $(L_{VBS,CPoLS}=2, C_{VBS,CPoLS}=1, T=1000)$ & 93.2265 & 88.1547 & 87.0614 & 57.9401 & 0.8760 & 0.9730 \\
$\textsc{VBS}$ $(L_{VBS,CPoLS}=2, C_{VBS,CPoLS}=2, T=1000)$ & 93.2473 & 89.4059 & 85.5792 & 56.1706 & 0.8745 & 0.9706 \\

